Large scale visual place recognition with sub-linear storage growth

Robotic and animal mapping systems share many of the same objectives and challenges, but differ in one key aspect: where much of the research in robotic mapping has focused on solving the data association problem, the grid cell neurons underlying maps in the mammalian brain appear to intentionally break data association by encoding many locations with a single grid cell neuron. One potential benefit of this intentional aliasing is both sub-linear map storage and computational requirements growth with environment size, which we demonstrated in a previous proof-of-concept study that detected and encoded mutually complementary co-prime pattern frequencies in the visual map data. In this research, we solve several of the key theoretical and practical limitations of that prototype model and achieve significantly better sub-linear storage growth, a factor reduction in storage requirements per map location, scalability to large datasets on standard compute equipment and improved robustness to environments with visually challenging appearance change. These improvements are achieved through several innovations including a flexible user-driven choice mechanism for the periodic patterns underlying the new encoding method, a parallelized chunking technique that splits the map into sub-sections processed in parallel and a novel feature selection approach that selects only the image information most relevant to the encoded temporal patterns. We evaluate our techniques on two large benchmark datasets with the comparison to the previous state-of-the-art system, as well as providing a detailed analysis of system performance with respect to parameters such as required precision performance and the number of cyclic patterns encoded.

==> tex/intro <==
\section{INTRODUCTION}
Recent years have witnessed tremendous success of autonomous systems with advanced mapping capabilities, enabling a robot or a self-driving car to accurately navigate itself within a known (or even unknown) environment. Such ability can be achieved thanks to strong developments in visual place recognition algorithms that allow the precise identification of locations throughout different seasons or weather conditions. The key paradigm behind the aforementioned algorithms is to learn a good representation, which can then be embedded into effective coding schemes.

However, most methods proposed in the literature focus mainly on improving query accuracy, while the storage requirements are \hl{of little interest}. As the size of training data increases -- the environment that the robot needs to navigate is expanded -- the storage size required by current algorithms also scales linearly to maintain the same accuracy.

A pioneer work in this research field can be relate to~\cite{yu2018rhythmic}, in which the authors proposed a novel encoding scheme inspired by recent findings on how the neurons of many mammals such as rodents behave~\cite{giocomo2007temporal} when it comes to recognizing places. By taking advantage of the grid cells, where each cell encodes a set of specific locations, they proposed a encoding algorithm that is capable of learning a map with high accuracy. Also, the storage requirements required by~\cite{yu2018rhythmic} scale up sub-linearly with the training data. However, there remain some drawbacks in~\cite{yu2018rhythmic} that need to be addressed.

In this work, inspired by~\cite{yu2018rhythmic}, we present a new encoding scheme that tackles some shortcomings in~\cite{yang2016towards}, with improved accuracy and lower storage requirements. Specifically, 
\begin{itemize}
        \item We present a new encoding algorithm that is able to handle large amount of training data, while the required storage scales sub-linearly with the number of scenes. In contrast to~\cite{yu2018rhythmic}, we allow the pattern periods to be chosen arbitrarily. This gives the user more freedom in fine-tuning the required storage that best matches the application requirements.
        \item To efficiently learn the patterns with our new encoding scheme, we introduce a novel feature selection approach, enabling us to extract the most valuable information in each pattern to encode. This leads to a drastic reduction in the amount of storage required, while the accuracy is maintained or improved compared to the results provided by~\cite{yu2018rhythmic}.
        \item Our algorithm is able to handle data with changing conditions with considerably good performance. Besides, different state-of-the-art representation learning can be used in our algorithm to further improve accuracy.
        \item We provide an implementation that makes use of GPU and multi-processing capabilities, allowing the handling of large amount of training data.
\end{itemize}



